A Stochastic Majorize-Minimize Subspace Algorithm for Online Penalized Least Squares Estimation

Stochastic approximation techniques play an important role in solving many problems encountered in machine learning or adaptive signal processing. In these contexts, the statistics of the data are often unknown a priori or their direct computation is too intensive, and they have thus to be estimated online from the observed signals. For batch optimization of an objective function being the sum of a data fidelity term and a penalization (e.g. a sparsity promoting function), Majorize-Minimize (MM) methods have recently attracted much interest since they are fast, highly flexible, and effective in ensuring convergence. The goal of this paper is to show how these methods can be successfully extended to the case when the data fidelity term corresponds to a least squares criterion and the cost function is replaced by a sequence of stochastic approximations of it. In this context, we propose an online version of an MM subspace algorithm and we study its convergence by using suitable probabilistic tools. Simulation results illustrate the good practical performance of the proposed algorithm associated with a memory gradient subspace, when applied to both non-adaptive and adaptive filter identification problems.

==> alphabet.tex <==
% Document LaTeX        GLB (25/05/94)
% Modification :        Gio (15/09/95)
%                       JI  (format Latex 2e, taille adaptative 22/03/99)
%                           (fonte blackboard 27/08/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\typeout{Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{(necessite les packages xspace, amsmath, bbm)}
\typeout{}

\RequirePackage{amsmath}
\RequirePackage{xspace}
\RequirePackage{bbm}
%\RequirePackage{amssymb}
%\RequirePackage{bbold}
%\RequirePackage{mathbbol}
%\RequirePackage{doublestroke}

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
%\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)
\def\sbl#1{\ensuremath{\mathbb{#1}}}

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}

% Complément intéressant...

\def\ellb{\sbmm{\ell}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}


% ALPHABET GREC GRAS italique, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}      \def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\varkappab   {{\sbmm{\varkappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}     \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}         \def\Xib       {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}         \def\Pib       {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}   \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib      {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib      {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}    \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{O}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS}
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}






==> jidef.tex <==

%\tiny\scriptsize\footnotesize\small\normalsize\large\Large\LARGE\huge\Huge

%\setlength{\abovedisplayskip}{6pt}         % Pour bricoler l'espace,
%\setlength{\belowdisplayskip}{6pt}         % Autour des equations...
%\setlength{\abovedisplayshortskip}{6pt}    % (Bon d'accord, je finasse)
%\setlength{\belowdisplayshortskip}{6pt}    % Pas d'improvisation!

% pour tasser la biblio: ajouter \setlength{\itemsep}{0pt} en deuxieme ligne du .bbl

\RequirePackage{accents} % e.g. \frown
\RequirePackage{amssymb} % e.g. \geqslant

\def\nnb{\nonumber}
\def\dd{\,\dD}                         % doit etre droit en francais
\def\leq{\leqslant}
\def\geq{\geqslant}
\renewcommand{\det}[1]{\bars{#1}}
\def\V{,\kern-.1em}  	% Virgule pour les nombres decimaux
%\def\V{.}              % Point pour les anglo-saxons
\def\e#1{.10^{#1}}      % Notation scientifique a la francaise
%\def\e#1{\rm{e}^{#1}}  % Notation scientifique anglo-saxonne

%\def\et{{\normalfont et }}
\def\et{{et}\ }
\def\numero{}
\def\editornames{(dir.)}
\def\editorname{(dir.)}
\def\eqname{équation~}
\def\eqnames{équations~}
\def\tabname{tableau~}
\def\tabnames{tableaux~}
\def\figname{figure~}
\def\fignames{figures~}
\def\chapname{chapitre~}
\def\chapnames{chapitres~}
\def\parname{pa\-ra\-gra\-phe~}
\def\parnames{pa\-ra\-gra\-phes~}
\def\sectname{section~}
\def\theoname{théorème~}
\def\gui#1{\<#1\>}
%\def\<{<<\,}\def\>{\,>>}
\def\<{\og}\def\>{\fg}
\def\ier{-ier\XS}
\def\iere{-ière\XS}
\def\ieme{-ième\XS}

\def\para{\cl{\btabu{c}$\ast$~~~$\ast$\\$\ast$\\[-.2cm]\etabu}}
\def\Separe{\medskip\cl{\rule{3cm}{.02cm}}}
\def\Fin{\cl{\rule{1.5cm}{.02cm}}\cl{\rule{.75cm}{.02cm}}}  % deux traits pour fin

%------------------------------------------------------------------
% Mise en commentaire rapide !
\def\rem#1{}                    % rem{bla bla bla}

\newenvironment{void}[1]
  {\begin{minipage}\white}
  {\end{minipage}}

\def\In{in }
\def\volume{vol.\,}
\def\PAGE{p.\,}
\def\PAGES{p.\,}
%\def\editionname{édition}

\newcommand{\tabref}[2][]{\tabname\ref{#2}{\normalfont#1}\XS}
\newcommand{\figref}[2][]{\figname\ref{#2}{\normalfont#1}\XS}
\newcommand{\refeq}[1]{\eqname(\ref{#1})\XS}
\newcommand{\refeqs}[1]{\eqnames(\ref{#1})\XS}
\def\chapref#1{\chapname\ref{#1}\XS}
\def\parref#1{\parname\ref{#1}\XS}
\def\parsref#1{\parnames\ref{#1}\XS}
\def\sectref#1{\sectname\ref{#1}\XS}
\def\refpage#1{\page\pageref{#1}\XS}
\def\reff{\XS\eqref}

\newcommand{\page}{p.~}
\newcommand{\pages}{pp.~}
%\def\nompage{p.\,}
%\def\nompages{pp.\,}
\def\numero{n\ensuremath{^{\circ}}}
\def\primo{\ensuremath{1^{\circ}}\XS}
\def\secundo{\ensuremath{2^{\circ}}\XS}
\def\tertio{\ensuremath{3^{\circ}}\XS}
\def\quatro{\ensuremath{4^{\circ}}\XS}

\def\B{\text{\large$\bullet$}}
\def\incirc#1{\pscirclebox[framesep=1pt]{\scriptsize#1}}
\def\incircp#1{\pscirclebox[framesep=1pt]{\tiny#1}}
\def\outcirc#1{\raisebox{-3pt}{\huge$\times$}\hspace*{-.45cm}\text{\incirc{#1}}}

\def\traitplein{\text{$\kern-1pt\frac{\kern5pt}{\kern7pt}\kern-2pt$}}
\def\tirets{\text{\kern-1pt-{}-{}-\kern-1pt}}
\def\pointilles{\text{$\cdot$$\cdot$$\cdot$\kern-1pt}}

\def\para{~\\[-.75cm]\bcc $\ast$~~~$\ast$\\$\ast$\ecc~\\[-.75cm]}

%-- Accolades, parenthèses, etc --------------------------------------
        
\def\pth#1{\left(#1\right)}                \def\stdpth#1{(#1)}
\def\acc#1{\left\{#1\right\}}              \def\stdacc#1{\{#1\}}
\def\cro#1{\left[#1\right]}                \def\stdcro#1{[#1]}
\def\croext#1{\left]#1\right[}             \def\stdcroext#1{]#1[}
\def\bars#1{\left|#1\right|}               \def\stdbars#1{|#1|}
\def\norm#1{\left\|#1\right\|}             \def\stdnorm#1{\|#1\|}
\def\scal#1{\left\langle#1\right\rangle}   \def\stdscal#1{\langle#1\rangle}
 
\def\bigpth#1{\bigl(#1\bigr)}              \def\biggpth#1{\biggl(#1\biggr)}
\def\bigacc#1{\bigl\{#1\bigr\}}            \def\biggacc#1{\biggl\{#1\biggr\}}
\def\bigcro#1{\bigl[#1\bigr]}              \def\biggcro#1{\biggl[#1\biggr]}
\def\bigcroext#1{\bigl]#1\bigr[}           \def\biggcroext#1{\biggl]#1\biggr[}
\def\bigbars#1{\bigl|#1\bigr|}             \def\biggbars#1{\biggl|#1\biggr|}
\def\bignorm#1{\bigl\|#1\bigr\|}           \def\biggnorm#1{\biggl\|#1\biggr\|}
\def\bigscal#1{\bigl\langle#1\bigr\rangle} \def\biggscal#1{\biggl\langle#1\biggr\rangle}

\def\Bigpth#1{\Bigl(#1\Bigr)}              \def\Biggpth#1{\Biggl(#1\Biggr)}
\def\Bigacc#1{\Bigl\{#1\Bigr\}}            \def\Biggacc#1{\Biggl\{#1\Biggr\}}
\def\Bigcro#1{\Bigl[#1\Bigr]}              \def\Biggcro#1{\Biggl[#1\Biggr]}
\def\Bigcroext#1{\Bigl]#1\Bigr[}           \def\Biggcroext#1{\Biggl]#1\Biggr[}
\def\Bigbars#1{\Bigl|#1\Bigr|}             \def\Biggbars#1{\Biggl|#1\Biggr|}
\def\Bignorm#1{\Bigl\|#1\Bigr\|}           \def\Biggnorm#1{\Biggl\|#1\Biggr\|}
\def\Bigscal#1{\Bigl\langle#1\Bigr\rangle} \def\Biggscal#1{\Biggl\langle#1\Biggr\rangle}

%------------------------------------------------------------------
\def\cl#1{\centerline{#1}} \def\eqcl#1{\cl{$\displaystyle#1$}} \def\eq#1{{$\displaystyle#1$}}

\def\nablab{\text{\boldmath$\nabla$}}
\def\wh#1{\widehat{#1}}    \def\wt#1{\widetilde{#1}}
\def\foo#1{{\text{\def\scad{-3}\tiny #1}}}
\def\T{^\tD}
%\def\T{^T}
\def\M{^{-1}}
\def\MT{^{-\tD}}
\def\+{^\dagger}
\def\I{\,|\,}           % "sachant" bien espacé pour les formules
\def\J{\mathop{\,;\,}}  % "point virgule" bien espacé pour les formules.
\def\w{,\thinspace}
\def\W{,\thickspace}
\def\ldotsv{,\,\ldots,\,}
\def\Exp#1{\exp\acc{#1}}
\def\Expp#1{e^{#1}}
\def\argmax{\mathop{\mathrm{arg\,max}}} % Mieux que \def\argmax{\arg\max}
\def\argmin{\mathop{\mathrm{arg\,min}}} % car l'indice est reparti
\def\Vect{\mathop{\text{Vect}}}
\def\Card{\mathrm{Card}}
\def\Circul#1{\mathrm{Circul}\{#1\}}
\def\toeplitz#1{\mathrm{T{\oe}plitz}\{#1\}}
\def\Id{\mathit{Id}}
\def\cste{\mathrm{cste}}
\def\trace{\mathrm{trace}}
\def\rang{{\mathrm{rang}}}
\def\Cov{\mathrm{Cov}}
\def\diag{{\mathrm{diag}}}
\def\Diag{\mathrm{Diag}}
\def\DIAG#1{\mathrm{Diag}\acc{#1}}
\def\Ker{\mathrm{Ker\,}}
\def\Img{\mathrm{Im\,}}
\def\Div{{\mathrm{div}}}
\def\FT#1{\protect\accentset{\frown}{#1}}
% Pour mettre un \No{} au-dessus d'une lettre (\TM, 02/97) (package{amsmath.sty})
%\def\rond#1{\overset{\kern-0.33em~_\circ}{#1}}
%\def\rondit[#1]#2{\overset{\kern#1~_\circ}{#2}}
\def\EL{\mathrm{EL}}
\def\esp{\ED\,}
\newcommand{\Esp}[2][]{\ED{_{#1}}\kern-2pt\cro{#2}}
%\def\Esp#1{\ED\kern-1pt\pth{#1}}
\def\stdEsp#1{\ED\stdcro{#1}}
%\def\EMQ{\mathit{EMQ}}
\def\var{\mathrm{var}\,}	\def\Var#1{\mathrm{var}\pth{#1}}	
\def\cov{\mathrm{cov}}		\def\Cov#1{\mathrm{cov}\kern-2pt\pth{#1}}
\def\egal{\kern-.5em=\kern-.5em}
\def\egdef{\stackrel{\Delta}{=}}
\newcommand{\imag}[1]{\mathrm{Im}\acc{#1}}
\newcommand{\reel}[1]{\mathrm{Re}\acc{#1}}
\newcommand{\impur}{\ensuremath{j}}

\def\sump{\mathop{\raisebox{-.3ex}{\text{\Large$\Sigma$}}}}
\def\intp{{\text{\small$\int$}}}
\def\prodp{\mathop{\raisebox{-.3ex}{\text{\Large$\Pi$}}}}
\newcommand{\fracp}[2]{\frac{\raisebox{-1pt}{$#1$}}{#2}}
\newcommand{\UNsur}[1]{\fracp{1}{#1}}
\def\demi{\UNsur{2}}
\def\ds{\displaystyle}
\def\ss{\scriptstyle}
\def\fracds#1#2{{\ds\frac{#1}{#2}}}
\def\fracts#1#2{{\ss\frac{#1}{#2}}}
\def\derpar#1#2{{\frac{\partial #1}{\partial #2}}}
\def\froc#1#2{{#1/#2}}     \def\fric#1#2{\frac1{#2}#1}
\def\derpor#1#2{{\froc{\partial #1}{\partial #2}}}
\def\parsec#1#2#3{{\frac{\partial^2 #1}{\partial #2\,\partial #3}}}
\def\parsecd#1#2{{\frac{\partial^2 #1}{{\partial #2}^2}}}
\def\porsec#1#2#3{{\froc{\partial^2 #1}{\partial #2\,\partial #3}}}
\def\porsecd#1#2{{\froc{\partial^2 #1}{{\partial #2}^2}}}
\def\pornd#1#2#3{{\froc{\partial^{#3} #1}{{\partial #2}^{#3}}}}
%\def\sur{\ensuremath{\kern-1pt/\kern-1pt}}
\def\diff#1#2{{\frac{\dd#1}{\dd#2}}}

%------------------------------------------------------------

\newsavebox{\fminibox}
\newlength{\fminilength}
\newenvironment{fminipage}[1][\linewidth]
  {\setlength{\fminilength}{#1}%-2\fboxsep-2\fboxrule%
   \begin{lrbox}{\fminibox}\begin{minipage}{\fminilength}}
  {\end{minipage}\end{lrbox}\noindent\fbox{\usebox{\fminibox}}}

\def\arrayp{\renewcommand{\arraystretch}{.7}\setlength{\arraycolsep}{2pt}}
\def\tabp{\renewcommand{\arraystretch}{.7}\setlength{\tabcolsep}{2pt}}

% Centre verticalement la colonne :
\def\cc#1{\setlength{\tabcolsep}{0pt}\btabu{c}#1\etabu}
\newcommand{\figc}[2][]
   {\setlength{\tabcolsep}{0pt}\btabu{c}\includegraphics[#1]{#2}\etabu}
   %{\setlength{\tabcolsep}{0pt}\btabu{c}\includegraphics[draft=true,#1]{#2}\etabu}
   %{\btabu{c}\small\texttt{\btabu{c}includegraphics[#1]\\\{\url{#2}\}\etabu}\etabu}

%\def\yaxis#1{\cc{\rotateleft{#1}}}
\def\ylabel#1{\cc{\rotateleft{#1}}}

\newlength{\vshift} \newlength{\hshift} % Pour hspace et vspace en pstricks

%\boite{length}{blabla} utilisable dans \caption... marche pas !
%\def\boite#1#2{#2\settowidth{\hshift}{#2}\addtolength{\hshift}{-#1}\hspace*{-\hshift}}
%\boite{blabla1}{blabla2} utilisable dans \caption
\def\boite#1#2{#2\settowidth{\hshift}{#1}\hspace*{\hshift}\settowidth{\hshift}{#2}\hspace*{-\hshift}}

%------------------------------------------------------------------

\def\UP#1{\uppercase{#1}}

\RequirePackage{ifthen}
\RequirePackage{calc}

\newcommand{\taille}[1][\scad]{%
\ifthenelse{#1 = -5}{}{}%
\ifthenelse{#1 = -4}{\tiny}{}%
\ifthenelse{#1 = -3}{\scriptsize}{}%
\ifthenelse{#1 = -2}{\footnotesize}{}%
\ifthenelse{#1 = -1}{\small}{}%
\ifthenelse{#1 = 0}{\normalsize}{}%
\ifthenelse{#1 = 1}{\large}{}%
\ifthenelse{#1 = 2}{\Large}{}%
\ifthenelse{#1 = 3}{\LARGE}{}%
\ifthenelse{#1 = 4}{\huge}{}%
\ifthenelse{#1 = 5}{\Huge}{}}

\newboolean{@serif}
\setboolean{@serif}{true}
\def\scad{-5} % scadefaultsize

\newcounter{taille}
\newcommand{\sca}[2][\scad]{\setcounter{taille}{#1}%
  \ifthenelse{\boolean{@serif}}
  {{\taille[\thetaille]\textsc{#2}}}
  {\setcounter{taille}{\value{taille}-1}{\uppercase{\taille[\thetaille]#2}}}}

%------------------------------------------------------------

\def\xbwh{\wh{\xb}{}}
%\def\qbwh{\kern1pt\wh{\kern-1pt\qb}{}}
\def\Xbwh{\kern1pt\wh{\kern-1pt\Xb}}
\def\Xvwh{\wh{\Xv}{}}
\def\Xvh#1{\Xvwh{}^{\foo{#1}}}
\def\xbh#1{\xbwh^{\foo{\normalfont#1}}}
\def\xh#1{\xwh^{\foo{\normalfont#1}}}
\def\xwh{\wh{x}{}}
\def\whtfx{{\stackrel{\raisebox{-5pt}{$\scriptscriptstyle\smash{\frown}$}}{\smash{\kern-.4pt \xwh}}}{}}
%\def\bvwh{\wh{\bv}{}}
%\def\hvwh{\wh{\hv}{}}
\def\bbwh{\wh{\bb}{}}
\def\hbwh{\wh{\hb}{}}
\def\thetabh#1{\wh{\thetab}{}^{\foo{\normalfont#1}}}

%------------------------------------------------------------------

\newcommand\unit[1]{\,\text{#1}\XS}
\def\Mo{\unit{Mo}\XS}
\def\MHz{\unit{MHz}\XS}
\def\kHz{\unit{kHz}\XS}
\def\Hz{\unit{Hz}\XS}
\def\cm{\unit{cm}\XS}
\def\mm{\unit{{mm}}\XS}
\def\ms{\unit{ms}\XS}
\def\dB{\unit{dB}\XS}
\def\sec{\unit{s}\XS}
\def\arcsec{\unit{arcsec}\XS}

\def\const{\textrm{const.}}
\def\SI{\text{si\:}}       \def\Si{\text{Si\:}}
\def\ET{\text{et\:}}       \def\OU{\text{ou\:}}
\def\ALORS{\text{alors\:}}
\def\DOU{\text{d'o\`u\:}}  \def\Ou{\text{o\`u\:}}
\def\QUAND{\text{quand\:}}
\def\POUR{\text{pour\:}}   \def\POURTOUT{\text{pour tout\:}}
\def\SC{\text{s.\,c.\:}}   \def\SOUSC{\text{sous contraintes\:}}
\def\SINON{\text{sinon}}
\def\AVEC{\text{avec\:}}
\def\DANS{\text{dans\:}}
\def\DONC{\text{donc}}

\def\adhoc{\textit{ad hoc}\XS}
\def\apost{\textit{a posteriori}\XS}
\def\Apost{\textit{A posteriori}\XS}
\def\APost{\textit{A Posteriori}\XS}
\def\post{\textit{posterior}\XS}
\def\Post{\textit{Posterior}\XS}
\def\afortio{\textit{a fortiori}\XS}
\def\Afortio{\textit{A fortiori}\XS}
\def\aprio{\textit{a priori}\XS}
\def\Aprio{\textit{A priori}\XS}
\def\Cad{C'est-\`a-dire\XS}
\def\cad{c'est-\`a-dire\XS}
\def\coeur{c{\oe}ur\XS}
\def\cf{\textit{cf.}\XS}
\def\cv{\textit{curriculum vit\ae}\XS}
\def\Cv{\textit{Curriculum vit\ae}\XS}
\def\CV{\textit{Curriculum Vit\ae}\XS}
\def\eg{\textit{e.g.,}\XS}
\def\andname{et\xspace}
\def\etal{{\itshape et coll.}}
\def\etc{{etc.}}
\def\etcoll{{\itshape et coll.}}
\def\idem{\textit{idem}\XS}
\def\ie{\textit{i.e.},\XS}
\def\IFF{\textit{if and only if}\XS}
\def\iid{i.i.d.\XS}
\def\infine{\textit{in fine}\XS}
\def\insit{\textit{in situ}\XS}
\def\inviv{\textit{in vivo}\XS}
\def\oeuvre{{\oe}uvre\XS}
\def\oeuvres{{\oe}uvres\XS}
\def\recto{\textit{recto}\XS}
\def\Toeplitz{T{\oe}plitz\XS}
\def\vav{vis-\`a-vis\XS}
\def\via{\textit{via}\XS}
\def\vic{\textit{vice-versa}\XS}
\def\verso{\textit{verso}\XS}
%\def\vitae{\textit{vit\ae}\XS}
\def\vs{\textit{vs}\XS}
\def\versus{\textit{versus}\XS}
\def\ssi{\textit{si et seulement si}\XS}
\def\strsen{\textit{stricto sensu}\XS}

%------------------------------------------------------------

\newcommand{\aic}[1][\scad]{\sca[#1]{aic}\XS}
\newcommand{\ar}[1][\scad]{\sca[#1]{ar}\XS}
\newcommand{\art}[1][\scad]{\sca[#1]{art}\XS}
\newcommand{\arma}[1][\scad]{\sca[#1]{arma}\XS}
\newcommand{\ma}[1][\scad]{\sca[#1]{ma}\XS}
%\newcommand{\bttb}[1][\scad]{\sca[#1]{bttb}\XS}
\newcommand{\bccb}[1][\scad]{\sca[#1]{bccb}\XS}
\newcommand{\bg}[1][\scad]{\sca[#1]{bg}\XS}
\newcommand{\dbg}[1][\scad]{\sca[#1]{dbg}\XS}
\newcommand{\cat}[1][\scad]{\sca[#1]{cat}\XS}
\newcommand{\ccd}[1][\scad]{\sca[#1]{ccd}\XS}
\newcommand{\cgm}[1][\scad]{\sca[#1]{cgm}\XS}
\newcommand{\cgmgg}[1][\scad]{\sca[#1]{cgmgg}\XS}
\newcommand{\clean}[1][\scad]{\sca[#1]{clean}\XS}
\newcommand{\clv}[1][\scad]{\sca[#1]{clv}\XS}
\newcommand{\clvh}[1][\scad]{\sca[#1]{clvh}}
\newcommand{\clvm}[1][\scad]{\sca[#1]{clvm}\XS}
\newcommand{\clpv}[1][\scad]{\sca[#1]{clpv}\XS}
\newcommand{\cnd}[1][\scad]{\sca[#1]{cnd}\XS}
\newcommand{\ct}[1][\scad]{\sca[#1]{ct}\XS}
\newcommand{\CP}[1][\scad]{\sca[#1]{cp}\XS}
\newcommand{\dse}[1][\scad]{\sca[#1]{dse}\XS}
\newcommand{\dsp}[1][\scad]{\sca[#1]{dsp}\XS}
\newcommand{\edp}[1][\scad]{\sca[#1]{edp}\XS}
\newcommand{\EM}[1][\scad]{\sca[#1]{em}\XS}
\newcommand{\EQM}{\sca{eqm}\XS}
\newcommand{\sem}[1][\scad]{\sca[#1]{sem}\XS}
\newcommand{\sirt}[1][\scad]{\sca[#1]{sirt}\XS}
\newcommand{\mvg}[1][\scad]{\sca[#1]{mvg}\XS}
\newcommand{\fft}[1][\scad]{\sca[#1]{fft}\XS}
\newcommand{\fpe}[1][\scad]{\sca[#1]{fpe}\XS}
\newcommand{\fk}[1][\scad]{\sca[#1]{fk}\XS}
\newcommand{\gc}[1][\scad]{\sca[#1]{gc}\XS}
\newcommand{\gcp}[1][\scad]{\sca[#1]{gcp}\XS}
\newcommand{\gcpc}[1][\scad]{\sca[#1]{gcpc}\XS}
\newcommand{\gnc}[1][\scad]{\sca[#1]{gnc}\XS}
\newcommand{\icd}[1][\scad]{\sca[#1]{icd}\XS}
\newcommand{\ig}[1][\scad]{\sca[#1]{ig}\XS}
\newcommand{\icm}[1][\scad]{\sca[#1]{icm}\XS}
\newcommand{\iwm}[1][\scad]{\sca[#1]{iwm}\XS}
\newcommand{\irm}[1][\scad]{\sca[#1]{irm}\XS}
\newcommand{\ldhy}[1][\scad]{\sca[#1]{l2h}y\XS}
\newcommand{\dldhy}[1][\scad]{\sca[#1]{dl2h}y\XS}
\newcommand{\ldlp}[1][\scad]{\sca[#1]{l2lp}\XS}
\newcommand{\lk}[1][\scad]{\sca[#1]{lk}\XS}
\newcommand{\map}[1][\scad]{\sca[#1]{map}\XS}
\newcommand{\mc}[1][\scad]{\sca[#1]{mc}\XS}
\newcommand{\mca}[1][\scad]{\sca[#1]{mca}\XS}
\newcommand{\mcmc}[1][\scad]{\sca[#1]{mcmc}\XS}
\newcommand{\mcreg}[1][\scad]{\sca[#1]{mcr}eg\XS}
\newcommand{\mdl}[1][\scad]{\sca[#1]{mdl}\XS}
\newcommand{\mem}[1][\scad]{\sca[#1]{mem}\XS}
\newcommand{\mmap}[1][\scad]{\sca[#1]{mmap}\XS}
\newcommand{\mpm}[1][\scad]{\sca[#1]{mpm}\XS}
\newcommand{\MP}[1][\scad]{\sca[#1]{mp}\XS}
\newcommand{\mV}[1][\scad]{\sca[#1]{mv}\XS}
\newcommand{\os}[1][\scad]{\sca[#1]{os}\XS}
\newcommand{\pC}[1][\scad]{\sca[#1]{pc}\XS}
\newcommand{\pocs}[1][\scad]{\sca[#1]{pocs}\XS}
\newcommand{\psf}[1][\scad]{\sca[#1]{psf}\XS}
\newcommand{\ri}[1][\scad]{\sca[#1]{ri}\XS}
\newcommand{\rif}[1][\scad]{\sca[#1]{rif}\XS}
\newcommand{\rp}[1][\scad]{\sca[#1]{rp}\XS}
\newcommand{\rls}[1][\scad]{\sca[#1]{rls}\XS}
\newcommand{\rsb}[1][\scad]{\sca[#1]{rsb}\XS}
\newcommand{\smlr}[1][\scad]{\sca[#1]{smlr}\XS}
\newcommand{\mmlr}[1][\scad]{\sca[#1]{mmlr}\XS}
\newcommand{\sage}[1][\scad]{\sca[#1]{sage}\XS}
\newcommand{\sar}[1][\scad]{\sca[#1]{sar}\XS}
\newcommand{\spect}[1][\scad]{\sca[#1]{spect}\XS}
\newcommand{\SF}[1][\scad]{\sca[#1]{sf}\XS}
\newcommand{\sq}[1][\scad]{\sca[#1]{sq}\XS}
\newcommand{\svd}[1][\scad]{\sca[#1]{svd}\XS}
\newcommand{\tcd}[1][\scad]{\sca[#1]{tcd}\XS}
\newcommand{\tep}[1][\scad]{\sca[#1]{tep}\XS}
\newcommand{\Th}[1][\scad]{\sca[#1]{th}\XS}
\newcommand{\tf}[1][\scad]{\sca[#1]{tf}\XS}
\newcommand{\tfd}[1][\scad]{\sca[#1]{tfd}\XS}
\newcommand{\tfr}[1][\scad]{\sca[#1]{tfr}\XS}
\newcommand{\tr}[1][\scad]{\sca[#1]{tr}\XS}
\newcommand{\tsvd}[1][\scad]{\sca[#1]{tsvd}\XS}
\newcommand{\us}[1][\scad]{\sca[#1]{us}\XS}
\newcommand{\vcg}[1][\scad]{\sca[#1]{vcg}\XS}

%\def\TF{\textrm{TF}\XS} \def\TFD{\foo{TFD}} \def\TFDD{\textrm{TFD}\XS}
%\def\tfd{TFD\XS}
%\def\fft{\foo{FFT}}
%\def\RSB{\textrm{RSB}\XS}

%------------------------------------------------------------

% Famous people - VIP

%\newcommand{\beaunom}[4][0]{{\taille[#1]#2 \uppercase{#3}}{\sca[#1]{#4}}\XS}
%\newcommand{\beaunom}[3][0]{#2 \sca[#1]{#3}\XS}

\newcommand{\MAL}[1][\scad]{Marc A\sca[#1]{llain}\XS}
\newcommand{\MBA}[1][\scad]{Michel B\sca[#1]{arlaud}\XS}
\newcommand{\LBE}[1][\scad]{Luigi B\sca[#1]{edini}\XS}
\newcommand{\ABL}[1][\scad]{Amandine B\sca[#1]{lanc}\XS}
\newcommand{\LBF}[1][\scad]{Laure B\sca[#1]{lanc}-F\sca[#1]{éraud}\XS}
\newcommand{\CBO}[1][\scad]{Charles A. B\sca[#1]{ouman}\XS}
\newcommand{\YBR}[1][\scad]{Yoram B\sca[#1]{resler}\XS}
\newcommand{\SBR}[1][\scad]{Stéphane B\sca[#1]{rette}\XS}
\newcommand{\DBR}[1][\scad]{David B\sca[#1]{rie}\XS}
\newcommand{\JFC}[1][\scad]{Jean--Fran\c{c}ois C\sca[#1]{ardoso}\XS}
\newcommand{\HCA}[1][\scad]{Hervé C\sca[#1]{arfantan}\XS}
\newcommand{\BCH}[1][\scad]{Bernard C\sca[#1]{halmond}\XS}
\newcommand{\FCH}[1][\scad]{Frédéric C\sca[#1]{hampagnat}\XS}
\newcommand{\LCH}[1][\scad]{Laurence C\sca[#1]{hatellier}\XS}
\newcommand{\PCI}[1][\scad]{Philippe C\sca[#1]{iuciu}\XS}
\newcommand{\GCI}[1][\scad]{Gabriela C\sca[#1]{iuperca}\XS}
\newcommand{\GCO}[1][\scad]{Guylaine C\sca[#1]{ollewet}\XS}
\newcommand{\PCO}[1][\scad]{Patrick C\sca[#1]{ombettes}\XS}
\newcommand{\CCO}[1][\scad]{Claude C\sca[#1]{omtat}\XS}
\newcommand{\MDA}[1][\scad]{Manuel D\sca[#1]{avy}\XS}
\newcommand{\ADE}[1][\scad]{Alexander H. D\sca[#1]{elaney}\XS}
\newcommand{\JDL}[1][\scad]{Jan De L\sca[#1]{eeuw}\XS}
\newcommand{\GDE}[1][\scad]{Guy D\sca[#1]{emoment}\XS}
\newcommand{\CDO}[1][\scad]{Christian D\sca[#1]{oncarli}\XS}
\newcommand{\FDU}[1][\scad]{Frédéric D\sca[#1]{ublanchet}\XS}
\newcommand{\SDU}[1][\scad]{Stéphanie D\sca[#1]{ubost}\XS}
\newcommand{\PDU}[1][\scad]{Patrick D\sca[#1]{uvaut}\XS}
\newcommand{\MFA}[1][\scad]{Marc F\sca[#1]{ayolle}\XS}
\newcommand{\DFA}[1][\scad]{Dario F\sca[#1]{arina}\XS}
\newcommand{\JFE}[1][\scad]{Jeffrey A. F\sca[#1]{essler}\XS}
\newcommand{\CFE}[1][\scad]{Cédric F\sca[#1]{évotte}\XS}
\newcommand{\MFI}[1][\scad]{Myriam F\sca[#1]{iani}\XS}
\newcommand{\IFI}[1][\scad]{Inbar F\sca[#1]{ijalkow}\XS}
\newcommand{\JJF}[1][\scad]{Jean-Jacques F\sca[#1]{uchs}\XS}
\newcommand{\LGA}[1][\scad]{Line G\sca[#1]{arnero}\XS}
\newcommand{\SGA}[1][\scad]{Stéphane G\sca[#1]{autier}\XS}
\newcommand{\DGE}[1][\scad]{Di G\sca[#1]{e}\XS}
\newcommand{\JFG}[1][\scad]{Jean--Fran\c{c}ois G\sca[#1]{iovannelli}\XS}
\newcommand{\SGO}[1][\scad]{Simon G\sca[#1]{odsill}\XS}
\newcommand{\EGO}[1][\scad]{Evans G\sca[#1]{ouno}\XS}
\newcommand{\YGO}[1][\scad]{Yves G\sca[#1]{oussard}\XS}
\newcommand{\JPG}[1][\scad]{Jean-Pierre G\sca[#1]{uédon}\XS}
\newcommand{\AHE}[1][\scad]{Alain H\sca[#1]{erment}\XS}
\newcommand{\DHU}[1][\scad]{David H\sca[#1]{unter}\XS}
\newcommand{\JID}[1][\scad]{Jér\^ome I\sca[#1]{dier}\XS}
\newcommand{\CLA}[1][\scad]{Christian L\sca[#1]{abat}\XS}
\newcommand{\JFL}[1][\scad]{Jean--Fran\c{c}ois L\sca[#1]{afay}\XS}
\newcommand{\JJL}[1][\scad]{Jean--Jacques L\sca[#1]{aurin}\XS}
\newcommand{\KLA}[1][\scad]{Kenneth L\sca[#1]{ange}\XS}
\newcommand{\RLE}[1][\scad]{Richard M. L\sca[#1]{eahy}\XS}
\newcommand{\GLB}[1][\scad]{Guy Le B\sca[#1]{esnerais}\XS}
\newcommand{\ELC}[1][\scad]{\'Eric Le C\sca[#1]{arpentier}\XS}
\newcommand{\MFL}[1][\scad]{Marie--Fran\c{c}oise L\sca[#1]{ucas}\XS}
\newcommand{\SMA}[1][\scad]{Salima M\sca[#1]{akni}\XS}
\newcommand{\TMA}[1][\scad]{Thierry M\sca[#1]{artin}\XS}
\newcommand{\VMA}[1][\scad]{Vincent M\sca[#1]{azet}\XS}
\newcommand{\OMI}[1][\scad]{Olivier M\sca[#1]{ichel}\XS}
\newcommand{\AMD}[1][\scad]{Ali M\sca[#1]{ohammad--}D\sca[#1]{jafari}\XS}
\newcommand{\SMO}[1][\scad]{Said M\sca[#1]{oussaoui}\XS}
\newcommand{\LMU}[1][\scad]{Laurent M\sca[#1]{ugnier}\XS}
\newcommand{\MNI}[1][\scad]{Mila N\sca[#1]{ikolova}\XS}
\newcommand{\NNO}[1][\scad]{Nicolas N\sca[#1]{ormand}\XS}
\newcommand{\JCP}[1][\scad]{Jean-Christophe P\sca[#1]{esquet}\XS}
\newcommand{\HPL}[1][\scad]{Hélène P\sca[#1]{iet}-L\sca[#1]{ahanier}\XS}
\newcommand{\NOU}[1][\scad]{Nadia O\sca[#1]{udjane}\XS}
\newcommand{\JBP}[1][\scad]{Jean-Baptiste P\sca[#1]{oline}\XS}
\newcommand{\ARI}[1][\scad]{Andrea R\sca[#1]{idolfi}\XS}
\newcommand{\KSA}[1][\scad]{Ken D. S\sca[#1]{auer}\XS}
\newcommand{\MSE}[1][\scad]{Myriam S\sca[#1]{ervières}\XS}
\newcommand{\HSN}[1][\scad]{Hichem S\sca[#1]{noussi}\XS}
\newcommand{\CSO}[1][\scad]{Charles S\sca[#1]{oussen}\XS}
\newcommand{\ITA}[1][\scad]{Ina T\sca[#1]{aralova}\XS}
\newcommand{\ETH}[1][\scad]{\'Eric T\sca[#1]{hiébaut}\XS}
\newcommand{\ATO}[1][\scad]{Anna T\sca[#1]{onazzini}\XS}
\newcommand{\TVE}[1][\scad]{Thomas V\sca[#1]{eit}\XS}
\newcommand{\CVO}[1][\scad]{Curtis R. V\sca[#1]{ogel}\XS}
\newcommand{\JZE}[1][\scad]{Josiane Z\sca[#1]{erubia}\XS}

\def\CNRS{Centre National de la Recherche Scientifique\XS}
%\newcommand{\cnrs}[1][\scad]{\sca[#1]{cnrs}\XS}

\def\UPS{Université de Paris-Sud\XS}
%\newcommand{\ups}[1][\scad]{\sca[#1]{ups}\XS}
%\newcommand{\ESE}[1][\scad]{\sca[#1]{supélec}\XS}
\def\LSS{Laboratoire des Signaux et Syst\`emes\XS}
\newcommand{\lss}[1][\scad]{\sca[#1]{l{\footnotesize 2}s}\XS}

%\newcommand{\tutelle}[1][\scad]{\cnrs[#1]~--~\ESE[#1]~--~\ups[#1]}
%\def\ALSS{\LSS~(\tutelle)\\\adresse}
%\def\ALSSun{\LSS (\tutelle) \adresse}
%\newcommand{\adresse}[1][\scad]{\ESE[#1], Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
%\def\adrshort{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex\XS}

\def\irccyn{Institut de recherche en communications et cybernétique\XS}
%\newcommand{\IRCCyN}[1][\scad]{\sca[#1]{ircc}y\sca[#1]{n}\XS}
\def\adts{Analyse et décision en traitement du signal\XS}
\def\adtsi{Analyse et décision en traitement du signal et de l'image\XS}
%\newcommand{\ADTS}[1][\scad]{\sca[#1]{adts}\XS}
%\newcommand{\ECN}[1][\scad]{\sca[#1]{ecn}\XS}
%\newcommand{\EMN}[1][\scad]{\sca[#1]{emn}\XS}
\def\UDN{Université de Nantes\XS}
%\newcommand{\udn}[1][\scad]{\sca[#1]{udn}\XS}
%\newcommand{\tutelle}[1][\scad]{\cnrs[#1]/\ECN[#1]/\EMN[#1]/\UDN}

%\RequirePackage{color}
\RequirePackage{pifont}
%\RequirePackage{/home/idier/tex/fonts/marvosym}	% ATTENTION : interferences bizarres (eg., \implies)
\RequirePackage[alpine]{ifsym}
\def\mail{}
\def\phone{~{\large \Telefon}~}%\ding{37}
\def\fax{~\smash{\normalsize\Faxmachine}~}
%\def\helvnormal#1{{\fontfamily{phv}\fontsize{10}{14pt}\selectfont #1}}
%\def\helvfoot  #1{{\fontfamily{phv}\fontsize{9}{14pt} \selectfont #1}}
%\def\helvscript#1{{\fontfamily{phv}\fontsize{8}{14pt} \selectfont #1}}

\newcommand{\edf}[1][\scad]{\sca[#1]{édf}\XS}
\newcommand{\cea}[1][\scad]{\sca[#1]{cea}\XS}
\newcommand{\hermes}{Hermes}
\newcommand{\onera}[1][\scad]{\sca[#1]{onera}\XS}
\def\EPM{\'Ecole polytechnique de Montréal\XS}
\def\SHFJ{Service Hospitalier Frédéric Joliot\XS}
\newcommand{\shfj}[1][\scad]{\sca[#1]{shfj}\XS}
\def\LENA{Laboratoire d'Encéphalographie et de Neurophysiologie Appliquée\XS}
%\newcommand{\lena}[1][\scad]{\sca[#1]{lena}\XS}
%\newcommand{\cnes}[1][\scad]{\sca[#1]{cnes}\XS}
\newcommand{\omp}[1][\scad]{\sca[#1]{omp}\XS}

\newcommand{\dea}[1][\scad]{\sca[#1]{dea}\XS}
\newcommand{\deaats}[1][\scad]{\sca[#1]{dea\,ats}\XS}
\newcommand{\deatis}[1][\scad]{\sca[#1]{dea\,tis}\XS}

%\newcommand{\ieee}[1][\scad]{\sca[#1]{ieee}\XS}
\newcommand{\ieee}{IEEE\XS}
\def\ieeeIP{\ieee Trans. on Image Processing}
\def\ieeeSP{\ieee Trans. on Signal Processing}
\def\ieeeIT{\ieee Trans. on Information Theory}
\def\ieeeSAP{\ieee Trans. on Speech and Audio Processing}
\def\ieeePAMI{\ieee Trans. on Pattern Analysis and Machine Intelligence}
\def\ICIP{IEEE Int. Conf. on Image Processing}
\def\GMIP{Graphical models and Image Processing}
\def\CRAS{Compte-rendus de l'Académie des sciences}
\def\TS{Traitement du signal}

